New Oracle-Efficient Algorithms for Private Synthetic Data Release

We present three new algorithms for constructing differentially private synthetic data---a sanitized version of a sensitive dataset that approximately preserves the answers to a large collection of statistical queries. All three algorithms are \emph{oracle-efficient} in the sense that they are computationally efficient when given access to an optimization oracle. Such an oracle can be implemented using many existing (non-private) optimization tools such as sophisticated integer program solvers. While the accuracy of the synthetic data is contingent on the oracle's optimization performance, the algorithms satisfy differential privacy even in the worst case. For all three algorithms, we provide theoretical guarantees for both accuracy and privacy. Through empirical evaluation, we demonstrate that our methods scale well with both the dimensionality of the data and the number of queries. Compared to the state-of-the-art method High-Dimensional Matrix Mechanism \cite{McKennaMHM18}, our algorithms provide better accuracy in the large workload and high privacy regime (corresponding to low privacy loss $\varepsilon$).

==> docs/adaptive_composition.tex <==

%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%% Adaptive composition
\section{zCDP Adaptive Parameter Composition}
In this section we show a technique to
do composition of zCDP-private mechanims with adaptively
choosen parameters.
The protocol \ref{alg:cdpadaparam} simulates the interaction
of against some adversary who chooses
the a sequence of privacy parameters $\rho_1, \ldots, \rho_k$.
Then we define a privacy filter \ref{def:filter} which on each
round takes as input the sequence of privacy parameters chosen by
the adversary and decides
whether the mechanism should stop or continue. If we run
some mechanim with a privacy filter such that if $\sum_{i=1}^k\rho_i > \rho$
then it stops then the mechanims would satisfy $\rho$-zCDP.

% \begin{algorithm}\label{algo:cdpadaparam}
% \KwIn{Adversary $\cA$, Rounds of interaction $k$, experiment parameter $b\in \{0,1\}$ }
% Select coin tosses $\cR_\cA^b$ for $\cA$ uniformly.\;
% \For{$i=1,\ldots, k$}{
% 	$\cA$ gives neighboring $x^{i,0}, x^{i,1}$,
% 	 parameter $(\eps_i)$, and $\cM_i$ that is
% 	  $(\eps_i)$-DP or $(\frac{1}{2}\eps_i^2)$-zCDP\;
% 	$\cA$ receives $A_i^b$
% }
% \textbf{Output: view }  $V^0 = \left(R_\cA, A_1^b, \ldots, A_k^b\right)$
% \caption{\adaParam($\cA, k, b$) \cite{rogers2016privacy}}
% \end{algorithm}


\begin{algorithm}[h]
\begin{algorithmic}
\caption{\adaParam($\cA, k, b$) \cite{rogers2016privacy}}
\label{alg:cdpadaparam}
\INPUT Adversary $\cA$, Rounds of interaction $k$, experiment parameter $b\in \{0,1\}$
\STATE Select coin tosses $R_\cA^b$ for $\cA$ uniformly
% , and
\FOR{$i \gets 1 $ \textbf{ to } $k$}
  \STATE $\cA$ gives neighboring $x^{i,0}, x^{i,1}$, parameter $\rho_i$, and $\cM_i$ that is $\rho$-zCDP
	% \STATE Add $q$ to $S_{t+1}$ with probability $\hat{\cQ}^{t+1}/\cQ^{t}$\;
	\STATE $\cA$ receives $A_i^b = \cM_i(x^{i,b})$
\ENDFOR
\OUTPUT  $V^b = \left(R_\cA^b, A_1^b, \ldots, A_k^b\right)$
\end{algorithmic}
\end{algorithm}

%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Definition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[Privacy Loss]
We define privacy loss for outcome $a$ and neighboring
datasets $x, x'$
\begin{align*}
\PrivLoss_\cM(a;x,x') =
\log\left( \frac{\pr{\cM(x) = a}}{\pr{ \cM(x') = a}} \right)
\end{align*}
\end{definition}
%


%%%%%%%%%%%%%%%%%%%%%%%
%% Def: zCDP Privacy Loss
%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[zCDP Privacy loss] Privacy loss
with respect to algorithm \adaParam
with input $(\cA, k, b)$ for a fixed view
$\nu = (r, a)$ where $r$ represents the random
coin tosses of $\cA$ and
$\nu_{<i} = (r, a_1, \ldots, a_{i-1})$. Each $\cM_i$
is $\rho(v_{<i})$-zCDP.
%
\[
\PrivLoss(\nu)
= \log\left( \frac{\pr{V^0 = \nu}}{\pr{ V^1 = \nu}} \right)
= \sum_{i=1}^k\log\left(\frac{\pr{\cM_i(x^{i,0}) = \nu_i |\nu_{<i}}}
{\pr{\cM_i(x^{i,1}) = \nu_i|\nu_{<i}}} \right)
= \sum_{i=1}^k \PrivLoss_{\cM_i}(\nu_{\leq i})
\]
\end{definition}



\begin{definition}[zCDP Privacy Filter]\label{def:filter}
A function
$F_{\rho}:\mathbb{R}_{\geq 0}^k
\longrightarrow \{\text{HALT},\text{CONT}\}$
is a valid privacy filter for $\rho>0$ if for
all adversaries $\cA$ in
$\adaParam(\cA, k, b)$ and all $\alpha>0$, when $v\sim V^0$, we
have
$$\PrivLoss(v) \leq \alpha\rho $$
\end{definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem: zCDP Simple Comp
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[zCDP Adaptive Parameter
Basic Composition]
For any $\rho>0$, $F_{\rho}$ is a valid
privacy filter where
\[
F_\rho(\rho_1, \ldots, \rho_k)=
\begin{cases}
\text{HALT} & \text{if } \sum_{i=1}^k \rho_i>\rho \\
\text{CONT } & \text{otherwise}
\end{cases}
\]
\end{theorem}
\begin{proof}
For any adversary $\cA$, and $k>0$.

Let view $V^0 = \adaParam(\cA, k, 0)$ and
$V^1 = \adaParam(\cA, k, 1)$.
Then for any realization of the view $v$ we have
and all $\alpha$

\begin{align*}
\PrivLoss(v)
% = \left| D_\alpha \left( V^0 ||V^1 \right) \right|
= \left| \sum_{i=1}^k D_\alpha
\left( \cM_{i}(x^{i,0}) ||
\cM_{i}(x^{i,1})  \right)
\right|
&\leq \alpha\sum_{i=0}^k \rho_i(v_{<i})
\end{align*}
where each $\rho_i(v_{<i})$ depends on all previous outcomes $v_{<i}$.
\end{proof}


==> docs/bounding.tex <==

We use a similar approach as in \cite{dann2017unifying} which uses the concept
of nice episodes but we modify their definition of nice episodes
to account for the noise the algorithm adds in order to preserve privacy.
Denote by $[T]$ the set of all episodes and again let $\sah \eqdefU (s,a,h)$.
Let the set of nice episodes $N\subset [T]$ be defined as
\begin{align*}
N = \left\{ t  : w_t(\sah) < w_{min} \text{ or }
 \frac{1}{4}\sum_{i<t} w_i(\sah) \geq \ln\frac{SAH}{\beta'} + 2\Eeps\right\}
\end{align*}
The number of suboptimal episodes is bounded by the number of suboptimal
nice episodes plus the number of non-nice episodes. In this section
we demonstrate how to bound each individually.


We use the following lemma \ref{lem:niceproperties} which
states some useful properties about nice episodes. Notably, we
get that on a nice episodes, if $\sah\notin L_t$ then
the private counter $\ntilt(\sah)$
is greater than two times the error bound of the counter $2\Eeps$.
%
%
%
%
First we bound the number of suboptimal nice episodes.
From now on we consider the gap $\Delta_t$ only on the nice
episodes.
Note that
$\conftilt(\sah) = (H+1)\phitilconfL{\sah}+\psitilconfL{\sah}$
if $\ntilt(\sah) \geq 2\Eeps$ otherwise
$\conftilt(\sah) = H$.
However, from lemma \ref{lem:niceproperties} we get that
if $\sah\notin L_t$
then $\ntilt(\sah) \geq 2\Eeps$. Therefore, if $t$ is a nice episode,
we can replace every $\conftilt(\sah)$ term in second term from the gap bound inequality
\ref{eq:main:gapII} and
the gap can be upper bounded as
%
\begin{align*}
\Delta_t \leq \frac{\alpha}{3} +
\Delta_{1,t} + \Delta_{2,t}
\end{align*}
%
where
\begin{align*}
\Delta_{1,t}= \sum_{\sah\notin L_t}w_t(\sah)(H+1)\phitilconfL{\sah}
\quad\quad\text{ and }\quad\quad \Delta_{2,t} =\sum_{\sah\notin L_t}w_t(\sah)\psitilconfL{\sah}
\end{align*}

%
% Then let $M_1$  be a subset of episodes where the gap $\Delta_{1,t}$
% is greater than $\alpha/3$, that is
% $M_1 = \{ t \in [T] : \Delta_{1,t} > \alpha/3 \}$. And correspongly for
% the gap $\Delta_{2,t}$ define the subset $M_2 = \{ t \in [T] : \Delta_{2,t} > \alpha/3 \}$.
%
%
Now we bound the number of nice episodes where term $\Delta_{2,t}$
is greater than $\alpha/3$. Recal that
$\psitilconfL{\sah} = \psitilconfR{\sah}$.
We use lemma \ref{lem:niceproperties} again that says that
w.p at leat $1-\beta$, if $t$ is a nice episode
and if $\sah\notin L_t$ then we have
 $\ntilt(\sah) \geq 2\Eeps$. Thus,
the following is true:
 $\frac{\Eeps^2}{\ntilt(\sah)^2} < \frac{\Eeps}{\ntilt(\sah)}$ on nice
 episode $t$. We can upper bound the gap $\Delta_{2,t}$ with
\begin{align*}
% \label{eq:main:gapPsiUpper}
\Delta_{2,t}
  &\leq \sum_{\sah\eqdefU (s,a,h) \notin L_t}w_t(\sah)
 (1+SH)\frac{10\Eeps}{\ntilt(\sah)}
\end{align*}
%
By lemma \ref{lem:mainrate} with $r=1$ we have that the number of
episodes where $\Delta_{t,2}>\tfrac{\alpha}{3}$ is at most
%
%
\begin{align}\label{eq:psiBound}
\frac{240\Eeps SAH}{\alpha}\polylog(S,A,H,1/\eps,1/\beta, 1/\alpha)
% \left| N \cap M_2 \right| \frac{\alpha}{3}
%  \leq \sum_{t\in N\cap M_2}\Delta_{2,t} \\
%  \leq 2SH(5\Eeps) \sum_{\sah\notin L_t}	\sum_{t\in N\cap M_2}
%     \frac{w_t(\sah)}{\sum_{i<t}w_t{\sah}} \\
% \leq 10S^2AH^2\Eeps\ln(T/w_{min})
\end{align}
%
% The third inequality is from
% $|L_k|\leq SAH$ and
% $\sum_{t\in N\cap M_1} \frac{w_t(\sah)}{\sum_{i<t}w_t(\sah)} \leq \ln(T/w_{min})$ which we get from lemma \ref{lem:lnbound} due to \cite{dann2017unifying} given below.
%

% Since $\Eeps \eqdefU \counterBound$, the number of nice episodes
% where $\Delta_{2,t}$ is greater than $\alpha/3$ is at most
% \begin{align}
% \label{eq:main:psiBound}
% \frac{90S^2AH^3}{\eps\alpha}\text{polylog}(T,S,A,H,(\beta')^{-1}, (\alpha)^{-1})
% \end{align}


\noindent For gap $\Delta_{1,t}$ we have
\begin{align*}
  \Delta_{1,t} \leq \sum_{x\notin L_t} w_t(\sah) (H+1)\phitilconfR{\sah}
\end{align*}
%
We  use lemma \ref{lem:mainrate} with $r=1$ to show that
$\Delta_{1,t}$ is greater than $\alpha/3$ on at most
\begin{align}
\label{eq:phiBound}
\frac{18SAH^4}{\alpha^2}\text{polylog}(S,A,H,(\beta')^{-1}, (\alpha)^{-1})
\end{align}
nice episodes.
Finally, the set of non-nice episodes is at most
\begin{align}\label{eq:notnice}
\frac{120S^2AH^4}{\alpha\eps}\polylog(S,A,H, 1/\beta)
\end{align}
%
$N^c + |N\cap M_1| + |N\cap M_2|$, which we have provided bounds in
for each term equations \ref{eq:notnice}, \ref{eq:phiBound},
\ref{eq:psiBound} gives that the number of $\alpha$-suboptimal
episodes is at most
\begin{align*}
O\left(
\left(\frac{S^2AH^4}{\eps\alpha} +\frac{SAH^3}{\alpha^2} \right) \polylog(T,S,A,H,(\beta')^{-1}, (\alpha)^{-1}) \right)
\end{align*}


==> docs/experiments_old2.tex <==
\section{Experiments on the Adult dataset}
\label{sec:experiments}
%
We evaluate the algorithms presented in this paper on two different datasets: the ADULT dataset from the UCI repository \cite{dua:2019} and the LOANS dataset. We focus on answering $5$-way marginals, with privacy budget $\eps$ taking value in $0.1, 0.15, 0.2, 0.25, 0.5$ and $1$. The datasets in our experiments are summarized in table \ref{table:summary}. To measure the accuracy of a synthetic dataset $\widehat{d}$  we used the max additive error over a set of queries $\{q_j\}$:
\begin{align*}
\textrm{err}(\widehat{D}) = \max_j \left|q_j(D)-q_j(\widehat{D})\right|
\end{align*}

In our implementation, algorithm \fem~ has hyperparameters $\eps_0$ and $\eta$ controlling the accuracy and the run time of the algorithm. We ran \fem~ on 20 different hyperparameter combinations and report the one with the minimum error in figures \ref{fig:errorI}, \ref{fig:errorII}, \ref{fig:queries}. The the range of hyperparameter we used is summarized in tables \ref{table:femparams} and \ref{table:dqparams}.

\begin{table}[h]
\caption{Datasets}
\label{table:summary}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Data set & Records & Attributes\\
\midrule
ADULT    & 48842 &  15  \\
LOANS    & 42535 &  48  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\begin{figure}
% {0.45\textwidth}
    % \vskip 0.1in
  \centering
  \includegraphics[width=\columnwidth]{results/adult.png}
  \caption{The ADULT dataset with 48,842 rows and 15 attributes. Running with
  The queries consist of $1,213,952$ $5$-way marginals. }
  \label{fig:errorI}
\end{figure}

\begin{figure}
% [b]{0.45\textwidth}
  % \vskip 0.1in
  \centering
  \includegraphics[width=\columnwidth]{results/loans.png}
  \caption{The LOANS dataset with $42,535$ rows and 48 attributes.
  The queries consist of $588,584$ $5$-way marginals.}
  \label{fig:errorII}
\end{figure}

We observed that among our three algorithms, $\fem$ consistently gets the best accuracy across different values of $\eps$. Therefore we focus on comparing \fem against HDMM, which is a state-of-the-art method. As shown in figure \ref{fig:errorI} and \ref{fig:errorII}, \fem~ scales better to the high privacy regime (low $\eps$ value). However, \hdmm~ has better runtime. From figure \ref{fig:queries}, we also see that \fem~ scales much better when the workload size if very large.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{results/adultqueries.png}
  \caption{Maximum error on the ADULT data set for different workload sizes. The workload sizes are 15, 60, 120, 180. The queries are the $5$-way marginals.}
  \label{fig:queries}
\end{figure}
%

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{results/loansqueries.png}
  \caption{Maximum error on the LOANS data set for different workload sizes. The workload sizes are 15, 30, 60, 120, 180. The queries are the $5$-way marginals.}
  \label{fig:queries}
\end{figure}

\paragraph{Optimazing over $k$-way Marginals} In our experiments, we optimize over a set of $k$-way marginal queries.
On each round $t$ the algorithm \fem~ takes as input a sequence of $t$ queries $(q_1, \ldots, q_t)$ and a random perturbation term $\sigma$ and solves the following  optimization problem

\begin{align*}
\argmax_x \left \{ \sum_{i=1}^{t-1} q_i(x) - \langle x, \sigma\rangle \right \}
\end{align*}

We represent a data record  by its one-hot binary encoding with dimension $d$, i.e.  $x\in \{0,1\}^d$. The $i^{th}$ $k$-way marginal query $q_i $ is associated with a binary vector $ w_i \in \{0,1\}^d$ with $\sum_{i=1}^d w_i = k$ which is an encoding of a conjunction over atributes in $x$, such that
\begin{align*}
  q_i(x) =
  \begin{cases}
    1 & \text{if } k = \sum_{j=1}^d x_j w_{i,j}  \\
    0 & \text{otherwise}
  \end{cases}
 \end{align*}
If $q_i$ is a negated query then
\begin{align*}
  q_i(x) =
  \begin{cases}
    0 & \text{if } k = \sum_{j=1}^d x_j w_{i,j}  \\
    1 & \text{otherwise}
  \end{cases}
\end{align*}

To implement the linear optimization oracle, we encode the optimization
problem as the following integer program
\begin{align*}
\max \sum_{i < t} c_i&
- \sum_{j=1}^d x_j \sigma_{j}\\
\mbox{s.t. }\sum_{j=1}^d x_j w_{i,j} \geq k c_i & \quad  \text{if } q_i \text{ is not negated}\\
\sum_{j=1}^d (1-x_j) w_{i,j} \geq c_i & \quad\text{if } q_i \text{ is  negated}
\end{align*}

We used the Gurobi solver for mixed-integer-programming to solve the
integer program.


\paragraph{Parameter Tunning}

In our implementation, algorithm \fem~ has hyperparameters $\eps_0$
and $\eta$. Both the accuracy and the run time of the algorithm depend
on how we choose these hyperparameters.  Table \ref{table:femparams}
contains a summary of \fem's parameters and the range of values that
we tested on.  The $\eta$ parameter is the scale of the random
objective perturbation term.  The data player samples a
synthetic dataset $\widehat{D}$ from the Follow The Perturbed Leader
distribution with parameter $\eta$ as in algorithm \ref{alg:fem}.  The
perturbation scale $\eta$ controls the rate of convergence of the
algorithm.  Setting this value too low can make the algorithm unstable
and leads to bad performance. If set too high, the solver in FTPL focuses too much on optimizing over the noise term.

The parameter $\eps_0$ corresponds to the privacy consumed on each
round by the exponential mechanism with the parameter $\eps_0$.  The goal is to find a query that maximizes the error on
$\widehat{D}$. Thus, the parameter $\eps_0$ controls the number of iterations. Again we face a trade-off in choosing
$\eps_0$, since setting this value too high can lead to too few
iterations giving the algorithm no chance to converge to a good
solution. If $\eps_0$ is too low, it can make the algorithm run too slow, and also it makes it hard for the query player's exponential mechanism to find queries with large errors.

\begin{table}[ht]
\caption{\fem~ hyperparameters.}
\label{table:femparams}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \begin{tabular}{lcccr}
\begin{tabularx}{\linewidth}{c XX }
\toprule
Param & Description & Range  \\
\midrule
$\eps_0$    & Privacy budget used per round &  0.001, 0.002, 0.003, 0.004, 0.1 \\
$\eta$    & Scale of noise for objective perturbation &  1, 2, 3, 4  \\
\bottomrule
\end{tabularx}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


For algorithm \dq~ and \dqrs~ we set parameters $\eta$ and $s$,
where $\eta$ is the update rate of MW and $s$ is the number of
samples from the distribution of MW. Table \ref{table:dqparams}
summarizes the range of parameters that we tried.

% \paragraph{Accuracy on small workloads}.
% Our first experiment is on the Adult dataset with a relati

\begin{table}[ht]
\caption{\dq~ and \dqrs~ hyperparameters.}
\label{table:dqparams}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \begin{tabular}{lcccr}
\begin{tabularx}{\linewidth}{c XX }
\toprule
Param & Description & Range  \\
\midrule
$\eta$    & Multiplicative Weight Rate &  0.2, 0.3, 0.4, 0.5, 0.6, 0.7 \\
$s$    & Number of samples from MW distribution &  10, 20, 30, 40, 50, 100 \\
\bottomrule
\end{tabularx}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% \begin{figure}[h]
% \vskip 0.1in
% \centering
% \includegraphics[width=0.6\columnwidth]{results/adult3.png}
% \caption{Maximum error and run time on Adult dataset for  62876
% $3$-way marginal queries.}
% \label{fig:errorI}
% \end{figure}
% %
% %

% \paragraph{Accuracy on large workloads}. We compare our proposed oracle

\paragraph{The implementation}   We ran the experiments on a machine with 4-core Opteron processor and 192 Gb of ram.

% \paragraph{Dynamic allocation of $\eps$}
% % The \dqrs~algorithm has many parameters.
%  For our theoretical analysis we have set these to mathematically convenient values. However, in our experimental implementation we take pains to optimize these. For this we employ concentrated differential privacy \cite{BunS16} to obtain sharp bounds on the accumulation of privacy loss over rounds. Furthermore, we dynamically allocate the privacy budget between rounds -- i.e., the parameters are re-optimized for each round based on the performance so far. To analyze the dynamic allocation of privacy budget, we extend the concentrated differential privacy framework to construct a so-called privacy filter \cite{rogers2016privacy}. These improvements do not make a difference in the asymptotic theoretical bounds, but are important for the practicality of our work.
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_icml2020.tex"
%%% End:


==> docs/rejection_sampling.tex <==
\section{Rejection Sampling}\label{sec:rs}

In this section, we present an improvement from the \DQ algorithm \cite{gaboardi2014dual}. In \DQ, the query player maintains a distribution over queries using Multiplicative Weights. But the algorithm can't directly release the distribution $\cQ^t$ proposed by MW during round $t$ because it depends on the private data. Instead, for each round $t$, it takes $s$ samples from $\cQ^t$ to form an estimate distribution $\widehat{\cQ^t}$. The data player then best-responds against $\widehat{\cQ^t}$. Our algorithm \RS improves the sampling step of \DQ. The basic idea is to apply the rejection sampling technique to generate a sample from $\cQ^t$ using samples obtained from the distribution in the previous round, i.e., $\cQ^{t-1}$. We show that by taking fewer samples from $\cQ^t$ for each round $t$, we use less of the privacy budget. The result is that the algorithm operates 
for more iterations and obtains better performance.

\subsection*{Privacy}
%
To enable our accounting of the privacy loss of the algorithm, we distinguish between ``good'' samples which are accepted in the rejection sampling step, and ``bad'' samples that are rejected, and require freshly sampling from $Q^{t+1}$. Both good and bad samples incur privacy loss from the decision whether to accept. 
%
\begin{lemma} \label{lem:good-samples}
The subroutine which accepts $q$ with probability $\hat{Q}^{t+1}_q /  Q^t_q = e^{-\eta-\gamma_t} \cdot \exp(-\eta A_D(x^t, q) )$ is $\eps$-differentially private for $\eps = \max\left\{\eta / n, \eta/\gamma_t n\right\}$.
\end{lemma}
%
%
Bad samples also incur privacy loss from sampling from the distribution $Q^t$. Just as in~\cite{GaboardiGHRW14}, we use the fact that this step can be viewed as an instantiation of the exponential mechanism with score function $\sum_{i = 1}^{t-1}(q(D) - q(x^i))$ to obtain:
%
\begin{lemma} \label{lem:bad-samples}
Sampling from $Q^{t}$ is $\eps$-differentially private for $\eps = 2\eta(t-1)/n$.
\end{lemma}
%
%
Finally, to control the cumulative privacy loss of the algorithm, we bound the number of bad samples.
%
\begin{theorem}
  \label{thm:rsprivacy}
  \dq with Rejection Sampling is $\rho$-CDP for
    \begin{align*}
    \rho &=  \frac{\eta^2 s}{n^2} (4T^{7/3} + 8 \eta T^3) = O\left(\frac{\log|\mathcal{X}| \cdot \log^{2+1/3}|\mathcal{Q}|}{n^2 \alpha^{4+2/3}}+\frac{\log|\mathcal{X}| \cdot \log^{3}|\mathcal{Q}|}{n^2 \alpha^{5}}\right).
  \end{align*}
%  \[
%    \eps = \frac{2 \eta (T-1)}{n} \cdot \left[ \sqrt{2s(T-1) \log(1/\delta)} + s(T-1) \left(
%        \exp\left( \frac{2 \eta (T-1)}{n} \right) - 1 \right) \right].
%  \]
\end{theorem}








